Accelerated nonlinear primal-dual hybrid gradient methods with applications to supervised machine learning

The linear primal-dual hybrid gradient (PDHG) method is a first-order method that splits convex optimization problems with saddle-point structure into smaller subproblems. Unlike those obtained in most splitting methods, these subproblems can generally be solved efficiently because they involve simple operations such as matrix-vector multiplications or proximal mappings that are fast to evaluate numerically. This advantage comes at the price that the linear PDHG method requires precise stepsize parameters for the problem at hand to achieve an optimal convergence rate. Unfortunately, these stepsize parameters are often prohibitively expensive to compute for large-scale optimization problems, such as those in machine learning. This issue makes the otherwise simple linear PDHG method unsuitable for such problems, and it is also shared by most first-order optimization methods as well. To address this issue, we introduce accelerated nonlinear PDHG methods that achieve an optimal convergence rate with stepsize parameters that are simple and efficient to compute. We prove rigorous convergence results, including results for strongly convex or smooth problems posed on infinite-dimensional reflexive Banach spaces. We illustrate the efficiency of our methods on $\ell_{1}$-constrained logistic regression and entropy-regularized matrix games. Our numerical experiments show that the nonlinear PDHG methods are considerably faster than competing methods.

==> unused.tex <==
\subsubsection{Support vector machines without offset}\label{subsec:svm}
For SVMs without offset, we seek to solve the primal minimization problem
%\todo{Add 1/m and fix the SVM algorithm...}
\begin{equation}\label{eq:svm_primal}
    \inf_{\bx \in \Rn} \left\{\frac{\lambda}{2}\normsq{\bx} + \frac{1}{m}\sum_{i=1}^{m} \max{\left(0, 1 + [\matr{A}\bx]_{i}\right)}\right\}.
\end{equation}
where $\matr{A}$ denotes the $m \times n$ real matrix whose columns are the features multiplied by the labels, that is, $A_{ij} = b_i(\Phi(\bx_i))_j$ with $b_{i} \in \{-1,+1\}$.
%Before proceeding, we wish to make two notes about the SVM problem~\eqref{eq:svm_primal}. First, in practice it is often more difficult to compute the matrix $\matr{A}$ directly than the kernel $K$ or its $m \times m$ kernel matrix $\matr{K} = [K(\bv_{i},\bv_{j})]_{ij}$ or the matrix product $\matr{A}\matr{A}^{*}$, the latter which can be computed via the kernel matrix:
%\begin{equation*}
%    [\matr{A}\matr{A}^{*}]_{ij} = b_{i}b_{j}K(\bv_{i},\bv_{j}).
%\end{equation*}
%Second, the quantity of interest to this problem is not the (unique) solution $\bx_{s}$ to problem~\eqref{eq:svm_primal}, but rather the hypothesis solution $\bv \mapsto \left\langle \bx_{s}, \bPhi(\bv) \right\rangle$. The accelerated nonlinear PDHG that we propose later will directly let us compute the hypothesis solution.
The dual problem for SVM optimization without offset is given by
\begin{equation}\label{eq:svm_dual}
\sup_{\by^{*} \in [0,1/m]^{m}} \left\{-\frac{1}{2\lambda}\normsq{\matr{A}^{*}\by^{*}} + \sum_{i=1}^{m} [\by^{*}]_{i} \right\}.
\end{equation}
The associated convex-concave saddle-point problem that we wish to solve is then
\begin{equation}\label{eq:svm_saddle}
    \inf_{\bx \in \Rn} \sup_{\by^{*} \in [0,1/m]^{m}} \left\{\frac{\lambda}{2}\normsq{\bx} + \left\langle \by^{*},\matr{A}\bx + \boldsymbol{1}_{m}\right\rangle \right\},
\end{equation}
where $\boldsymbol{1}_{m}$ denotes the $m$-dimensional vector whose entries are equal to 1. Due to the strong convexity of the primal problem~\eqref{eq:svm_primal}, the saddle-point problem~\eqref{eq:svm_saddle} admits at least one saddle point. If $(\bx_{s},\by_{s}^{*})$ is a saddle point of~\eqref{eq:svm_saddle}, then $\bx_{s}$ is the unique global minimum of the primal problem~\eqref{eq:svm_primal} and $\by_{s}^{*}$ is a global minimum of the dual problem~\eqref{eq:dual_prob}. Moreover, the saddle point $(\bx,\by_{s}^{*})$ satisfies the optimality conditions
\begin{equation}\label{eq:svm_opt-conds}
    -\matr{A}^{*}\by_{s}^{*} = \lambda \bx_{s} \quad \mathrm{and} \quad [\by_{s}^{*}]_{i} \in 
    \begin{dcases}
    0 \quad &\mathrm{if}\, [\matr{A}\bx_{s}]_i < -1, \\
    [0,1] \quad &\mathrm{if}\, [\matr{A}\bx_{s}]_i = -1, \\
    1 \quad &\mathrm{if}\, [\matr{A}\bx_{s}]_i > -1.
    \end{dcases}
    \quad \mathrm{for}\, i \in \{1,\dots,m\}.
\end{equation}



\subsubsection*{Accelerated nonlinear PDHG algorithm}
We propose to compute the solution of SVM optimization problem~\eqref{eq:svm_primal} using the accelerated nonlinear PDHG algorithm~\eqref{eq:accI_pdhg_alg} with the following choice of norms and Bregman functions:
\[
\normx{\cdot} = \normtwo{\cdot}, \quad \normys{\cdot} = \normone{\cdot}, \quad \phix = \frac{1}{2}\normsq{\cdot}, \quad \text{and} \quad \phiys = \frac{1}{4}\psi,
\]
where $\psi$ is, up to a factor of $1/4$, the average negative sum of $m$ binary entropy terms~\eqref{eq:binary-entropy}. The latter induces the Bregman divergence $D_{\psi}\colon [0,1/m]^{m} \times (0,1/m)^{m} \to \R$ given by~\eqref{eq:entropy-bregman}. With these choices, assumptions (A1)-(A5) hold. In particular, assumption (A5) holds because the Bregman function $\phiys$ is 1-strongly convex with respect to the $\ell_1$ norm. Moreover, the induced operator norm is the maximum $\ell_2$ norm of the rows of $\matr{A}$, which for the SVM optimization problem~\eqref{eq:svm_primal} is given by the largest Euclidean norm of the feature mapping among all samples $\bv_i$, i.e.,
\[
\normop{\matr{A}} = \sup_{\normtwo{\bx} = 1}\norminf{\matr{A}\bx} = \max_{i \in \{1,\dots,m\}} \sqrt{\sum_{j=1}^{n}A_{ij}^{2}} = \max_{i \in \{1,\dots,m\}} \normtwo{\bPhi(\bv_i)} = \max_{i \in \{1,\dots,m\}} \sqrt{\left|K(\bv_{i},\bv_{i})\right|}.
\]
The strong convexity parameter is $\gamma_{g} = \lambda$. Given $\theta_{0} \in (0,1)$, $\sigma_{0} = \lambda/(2\normop{\matr{A}}^2)$, $\tau_{0} = 2/\lambda$, $\bx_{0} \in \Rn$, and $\by^{*}_{-1} = \by^{*}_{0} \in (0,1)^m$, the accelerated nonlinear PDHG algorithm~\eqref{eq:accI_pdhg_alg} for the SVM optimization problem~\eqref{eq:svm_primal} consists of the iterations
\[
\begin{alignedat}{1}
    \bx_{k+1} &= \argmin_{\bx \in \Rn} \left\{\frac{\lambda}{2}\normsq{\bx} + \left\langle \by_{k}^{*} + \theta_{k}(\by_{k}^{*} - \by_{k-1}^{*}), \matr{A}\bx \right\rangle + \frac{1}{2\tau_{k}}\normsq{\bx-\bx_{k}}\right\} \\,
    \by_{k+1}^{*} &= \argmax_{\by^{*} \in [0,1/m]^{m}} \left\{\left\langle\by^{*},\matr{A}\bx_{k+1} + \boldsymbol{1}_{m}\right\rangle - \frac{1}{\sigma_{k}}D_{\psi}(\by^{*},\by^{*}_{k})\right\} \\
    \btheta_{k+1} &= 1/\sqrt{1 + \lambda\tau_{k}}, \quad \tau_{k+1} = \theta_{k+1}\tau_{k}, \quad \mathrm{and} \quad \sigma_{k+1} = \sigma_{k}/\theta_{k+1},
\end{alignedat}
\]

The updates $\bx_{k+1}$ and $\by^{*}_{k+1}$ can both be computed exactly. For the first update, a short calculation gives
\[
\bx_{k+1} = \left(\bx_{k} - \tau_{k}\matr{A}^{*}(\by_{k}^{*} + \theta_{k}(\by_{k}^{*} - \by_{k-1}^{*}))\right)/(1+\lambda\tau_{k}).
\]
% TODO: Update to kernel logistic regression. Also update to 
As for kernel ridge regression it is generally more difficult to compute the matrix $\matr{A}$ directly than the kernel $K$ or its $m \times m$ kernel matrix $\matr{A}\matr{A}^{*}$ given component-wise by $  [\matr{A}\matr{A}^{*}]_{ij}= b_{i}b_{j}K(\bv_{i},\bv_{j})$. To bypass this issue, define the auxiliary variable $\bu_{k} = \matr{A}\bx_{k}$ and multiply the update $\bx_{k+1}$ by the matrix $\matr{A}$ to get the update
\[
\bu_{k+1} = \left(\bu_{k} - \tau_{k}\matr{A}\matr{A}^{*}(\by_{k}^{*} + \theta_{k}(\by_{k}^{*} - \by_{k-1}^{*}))\right)/(1+\lambda\tau_{k}),
\]
The update in $\by_{k+1}^{*}$ depends only on $\bx_{k+1}$ through the matrix-vector product $\matr{A}\bx_{k+1}$, so we can substitute this product for $\bu_{k+1}$. Crucially, we can avoid computing the initial vector $\bu_{0} = \matr{A}\bx_{0}$ by setting $\bx_{0} = \boldsymbol{0}$.

For the second update, define the auxiliary variable $\bv_{k}$ component wise by
\[
[\bv_{k}]_{i} = \log\left(m[\by_{k}^{*}]_{i}/(1-m[\by_{k}^{*}]_{i})\right).
\]
Then with the auxiliary update
\[
\bv_{k+1} = \bv_{k} + 4\sigma_{k}(\matr{A}\bx_{k+1} + \boldsymbol{1}_{m})/m
\]
we get
\[
[\by_{k+1}]_{i} = 1/(m+m\exp{(-[\bv_{k}]_{i})})
\]
for $i \in \{1,\dots,m\}$.

In summary, our accelerated nonlinear PDHG algorithm for solving the SVM optimization problem is as follows. Let $\theta_{0} \in (0,1)$, $\sigma_{0} = \lambda/(2\normop{\matr{A}}^2)$, $\tau_{0} = 2/\lambda$, $\bu_{0} = \boldsymbol{0}$, and $\by^{*}_{-1} = \by^{*}_{0} \in (0,1)^m$. Then iterate
\begin{equation}\label{eq:alg_svm}
\begin{dcases}
    \bu_{k+1} &= \left(\bu_{k} - \tau_{k}\matr{A}\matr{A}^{*}(\by_{k}^{*} + \theta_{k}(\by_{k}^{*} - \by_{k-1}^{*}))\right)/(1+\lambda\tau_{k}), \\
    \bv_{k+1} &= \bv_{k} + 4\sigma_{k}(\matr{A}\bx_{k+1} + \boldsymbol{1}_{m})/m, \\
    [\by_{k+1}]_{i} &= 1/(m+m\exp{(-[\bv_{k}]_{i})}), \\
    \theta_{k+1} &= 1/\sqrt{1 + \lambda\tau_{k}}, \quad \tau_{k+1} = \theta_{k+1}\tau_{k}, \quad \mathrm{and} \quad \sigma_{k+1} = \sigma_{k}/\theta_{k+1},
\end{dcases}
\end{equation}
until convergence. The matrix product $\matr{A}\matr{A}^{*}$ can be calculated with the kernel via $\matr{A}\matr{A}^{*}]_{ij}= b_{i}b_{j}K(\bv_{i},\bv_{j})$. Note that all parameters and updates can be performed in $O(m^2)$ operations. According to Prop.~\ref{prop:acc_sq_algI} and the optimality conditions~\eqref{eq:svm_opt-conds}, we have the limits 
\[
 \lim_{k \to +\infty} \bu_{k} = \matr{A}\bx_{s} \quad \mathrm{and} \quad \lim_{k \to +\infty} \normtwo{\matr{A}\matr{A}^{*}\by_{k}^{*} + \lambda\bu_{k}} = 0,
\]
the latter which can serve as a convergence criterion.

---


\subsubsection{Elastic net linear regression}\label{subsec:enrlr}
Elastic net linear regression is a supervised learning algorithm for regression and for identifying important features in data sets. More precisely, suppose we receive $m$ independent samples, each comprising an $n$-dimensional vector of features and a response variable. The samples are encoded in an $m \times n$ real matrix $\matr{A}$ whose columns are the features and a response vector $\bb \in \Rm$. The primal problem for elastic net linear regression is then
\begin{equation}\label{eq:enrlr_primal}
\inf_{\bx \in \Rn} \left\{\lambda\left(\alpha\normone{\bx} + \frac{1-\alpha}{2}\normsq{\bx}\right) + \frac{1}{2m}\normsq{\matr{A}\bx - \bb} \right\},
\end{equation}
where $\lambda > 0$ is a tuning parameter and $\alpha \in (0,1)$ is a fixed hyperparameter. The regularizer $\bx \mapsto \lambda (\alpha \normone{\bx} + (1-\alpha)\normsq{\bx}/2)$ is called the elastic net~\cite{zou2005regularization}. \todo{I probably don't need to describe these penalties in detail... Revision for the whole section.}
It is a compromise between the ridge penalty ($\alpha = 0$)~\cite{hoerl1970ridge} and the lasso penalty ($\alpha = 1$)~\cite{tibshirani1996regression}. The elastic net penalty regularizes the linear regression model in three ways. First, it ensures that the linear regression problem~\eqref{eq:enrlr_primal} has a unique solution. Second, the squared $\ell_2$-norm shrinks the coefficients of correlated predictor variables toward each other (and zero), which alleviates negative correlation effects (e.g., high variance) between highly correlated predictor variables. Third, the $\ell_1$-norm promotes sparsity in the solution of~\eqref{eq:enrlr_primal}; that is, the global minimum of~\eqref{eq:enrlr_primal} has a number of entries that are identically zero~\cite{Foucart2013,el2020comparative,zanon2020sparse}. The non-zero entries are identified as the important predictor variables, and the zero entries are discarded. The number of non-zero entries itself depends on the value of the fixed hyperparameter $\alpha$ and the tuning parameter $\lambda$. 

In terms of the abstract primal problem~\eqref{eq:primal_prob}, we have 
\[
\xcal \in \Rn, \quad \bx \mapsto g(\bx) = \lambda\left(\alpha\normone{\bx} + \frac{1-\alpha}{2}\normsq{\bx}\right), \quad \mathrm{and} \quad \by \mapsto h(\by) = \frac{1}{2m}\normsq{\by - \bb}.
\]
To state the dual problem for elastic net linear regression, we need to compute the convex conjugate of the elastic net penalty:
\[
\begin{alignedat}{1}
g^{*}(\bx^{*}) &= \sup_{\bx \in \Rn} \left\{\left\langle \bx^{*},\bx \right\rangle - \lambda\left(\alpha\normone{\bx} + \frac{1-\alpha}{2}\normsq{\bx}\right) \right\} \\
&= \frac{1}{2\lambda(1-\alpha)}\normsq{\bx^{*}} - \inf_{\bx^{*} \in \Rn} \left\{\frac{\alpha}{1-\alpha}\normone{\bx} + \frac{1}{2}\normsq{\bx-\bx^{*}/(\lambda(1-\alpha))}\right\}.
\end{alignedat}
\]
The unique minimum to the infimum problem above can be expressed in terms of the soft thresholding operator~\cite{daubechies2004iterative,figueiredo2001wavelet,lions1979splitting}, defined for $j \in \{1.\dots,n\}$ and $\beta > 0$ by
\[
(\mathrm{shrink}_{1}(\bx^{*},\beta))_{j} = \begin{dcases}
    x^{*}_{j} - \beta &\quad \mathrm{if}\, x^{*}_{j} > \beta, \\
    0 &\quad \mathrm{if}\, |x^{*}_{j}| < \beta, \\
    x^{*}_{j} + \beta &\quad \mathrm{if}\, x^{*}_{j} < -\beta.
\end{dcases}
\]
The dual problem is therefore
\begin{equation}\label{eq:enrlr_dual}
\sup_{\by^{*} \in \Rm} \left\{\frac{1}{2\lambda(1-\alpha)}\normsq{-\matr{A}^{*}\by^{*}} - \mathrm{shrink}_{1}\left(\frac{-\matr{A}^{*}\by^{*}}{\lambda(1-\alpha)},\frac{\alpha}{1-\alpha}\right) - \left\langle\by^{*},\bb \right\rangle - \frac{m}{2}\normsq{\by^{*}}\right\}.
\end{equation}
In terms of the abstract dual problem~\eqref{eq:dual_prob}, we have 
\[
\ycals = \Rm, \quad \bx^{*} \mapsto g^{*}(\bx^{*}) = \frac{1}{2\lambda(1-\alpha)}\normsq{\bx^{*}} - \mathrm{shrink}_{1}\left(\frac{\bx^{*}}{\lambda(1-\alpha)},\frac{\alpha}{1-\alpha}\right),
\]
and
\[
\by^{*} \mapsto h^{*}(\by^{*}) = \left\langle \by^{*},\bb \right\rangle + \frac{1}{2}\normsq{\by^{*}}.
\]
The associated convex-concave saddle-point problem that we wish to solve is then
\begin{equation}\label{eq:enrlr_saddle}
    \inf_{\bx \in \Rn} \sup_{\by^{*} \in \Rm} \left\{\lambda\left(\alpha\normone{\bx} + \frac{1-\alpha}{2}\normsq{\bx}\right) + \left\langle \by^{*},\matr{A}\bx - \bb \right\rangle - \frac{m}{2}\normsq{\by^{*}} \right\}.
\end{equation}
Due to the strong convexity of the primal problem~\eqref{eq:enrlr_primal} and strong concavity of the dual problem~\eqref{eq:enrlr_dual}, the convex-concave saddle-point problem~\eqref{eq:enrlr_saddle} has a unique saddle point $(\bx_{s},\by_{s}^{*}) \in \Rn \times \Rm$. Here $\bx_{s}$ and $\by_{s}^{*}$ are the unique solutions to the primal and dual problems above. They satisfy the optimality conditions
\begin{equation}\label{eq:enrlr_opt-conds}
    -\matr{A}^{*}\by^{*}_{s} - \lambda(1-\alpha)\bx_{s} \in \lambda\alpha \partial \normone{\bx_{s}}  \quad \mathrm{and} \quad \by^{*}_{s} = \frac{1}{m}(\matr{A}\bx_{s} - \bb).
\end{equation}
Unlike kernel ridge regression, $\bx_{s}$ and $\by_{s}$ have no known closed-form solutions when $\alpha \in (0,1)$.

\subsubsection*{Accelerated nonlinear PDHG algorithm}
We propose to compute the solution of the elastic net linear regression problem using the accelerated nonlinear PDHG algorithm~\eqref{eq:accIII_pdhg_alg} with the following choice of norms and Bregman functions:
\[
\normx{\cdot} = \normone{\cdot}, \quad \normys{\cdot} = \normtwo{\cdot}, \quad \phix = \frac{n}{2}\normsq{\cdot}, \quad \mathrm{and} \quad \phiys = \frac{1}{2}\normsq{\cdot}.
\]
With these choices, assumptions (A1)-(A5) hold. In particular, assumption (A5) holds because of the norm equivalence $\sqrt{n}\normtwo{\bx} \geqslant \normone{\bx}$:
\[
\begin{alignedat}{1}
\phix(\bx) - \frac{1}{2}\normone{\bx}^{2} &= \frac{n}{2}\normsq{\bx} - \frac{1}{2}\normone{\bx}^{2} \\
&\geqslant \frac{1}{2}\normone{\bx}^{2} - \frac{1}{2}\normone{\bx}^{2} \\
&\geqslant 0.
\end{alignedat}
\]
Moreover, the induced operator norm~\eqref{eq:operator_norm} is the maximum $\ell_2$ norm of the columns of $\matr{A}$:
\[
\normop{\matr{A}} = \sup_{\normone{\bx} = 1}\normtwo{\matr{A}\bx} = \max_{j \in \{1,\dots,n\}} \sqrt{\sum_{i=1}^{m}A_{ij}^{2}}.
\]
Note that in elastic net linear regression, the columns of the matrix $\matr{A}$ are generally standardized and normalized, and the value of the operator norm will reflect this. The strong convexity parameters are $\gamma_g = \lambda(1-\alpha)/n$ and $\gamma_{h^*} = m$, and the stepsize parameters $\theta$, $\tau$, and $\sigma$ are accordingly
\[
\theta = 1 - \frac{\lambda(1-\alpha)m}{2n\normop{\matr{A}}^2}\left(\sqrt{1 + \frac{4n\normop{\matr{A}}^2}{\lambda(1-\alpha)m}} - 1\right), \quad \tau = \frac{n(1-\theta)}{\lambda(1-\alpha)\theta}, \quad \mathrm{and} \quad \sigma = \frac{1-\theta}{m\theta}.
\]
The accelerated nonlinear PDHG algorithm for the ridge regression problem and choice of norms and Bregman functions is then
\begin{equation}\label{eq:alg_enrlr}
    \begin{dcases}
    \bx_{k+1} &= \argmin_{\bx \in \Rn} \left\{\lambda\left(\alpha\normone{\bx} + \frac{1-\alpha}{2}\normsq{\bx}\right) + \left\langle \by_{k}^{*} + \theta(\by_{k}^{*} - \by_{k-1}^{*}), \matr{A}\bx \right\rangle + \frac{n}{2\tau}\normsq{\bx-\bx_{k}}\right\} \\
    &= \mathrm{shrink}_{1}\left(\frac{\tau\matr{A}^{*}(\by_{k}^{*} + \theta(\by_{k}^{*} - \by_{k-1}^{*}))-n\bx_{k}}{n + \tau\lambda(1-\alpha)},\frac{\tau\lambda\alpha}{n + \tau\lambda(1-\alpha)}\right), \\
    \by_{k+1}^{*} &= \argmin_{\by^{*} \in \Rm} \left\{\frac{m}{2}\normsq{\by^{*}} - \left\langle \by^{*}, \matr{A}\bx_{k+1} - \bb\right\rangle + \frac{1}{2\sigma}\normsq{\by^{*} - \by_{k}^{*}}\right\}\\
    &= \frac{\by_{k}^{*} + \sigma(\matr{A}\bx_{k+1} - \bb)}{1+m\sigma}.
    \end{dcases}
\end{equation}
where $\bx_{0} \in \Rn$ and $\by_{-1} = \by_{0} \in \Rm$ are (free) initial values. Note that all parameters and updates can be performed in $O(mn)$ operations. According to Prop.~\ref{prop:acc_sq_algII_var} and the optimality conditions~\eqref{eq:enrlr_opt-conds}, we have the limits 
\[
\lim_{k \to +\infty} \bx_{k} = \bx_{s}, \quad \lim_{k \to +\infty} \by_{k}^{*} = \by_{s}^{*}, \quad \mathrm{and} \lim_{k \to +\infty} \normtwo{m\by_{k}^{*} - (\matr{A}\bx_{k} - \bb)} = 0,
\]
the latter which can serve as a convergence criterion. % TODO: CHECK

\begin{comment}
\subsection{Support vector machines without offset}
For this experiment, we used a quadratic polynomial kernel:
\[
K(\bv,\bv') = \left(\left\langle \bv,\bv'\right\rangle + \frac{1}{2}\right)^{2}
\]
and the dimensions $(m,d) = (1000, 100000)$, $(m,d) = (2500, 40000)$, and $(m,d) = (10000, 10000)$ for the samples $(\bv_{1},\dots,\bv_{m})$. The dimension of the primal problem~\eqref{eq:svm_primal} is $n = {d + 2 \choose 2}$. For each pair $(m,d)$, we used the correlation coefficient $r \in \{0.25,0.75\}$, for a total of six simulations. In each simulation, we generated 100 values of $\lambda$ logarithmically spaced from $10^5$ to $10^{-5}$ using the MATLAB command \emph{logspace(5,5,100)}. We then solved the kernel ridge regression problem~\eqref{eq:svm_primal} sequentially for each $\lambda_{l}$ with our implementation of the nonlinear PDHG algorithm~\eqref{eq:alg_svm} and FISTA using the dual solution found for~\eqref{eq:svm_primal} with tuning parameter $\lambda_{l}$ as the initial dual solution for~\eqref{eq:svm_primal} with tuning parameter $\lambda_{l+1}$. The initial values $\by_{-1}^{*} = \by_{0}^{*} = \boldsymbol{\bb}$ were used for solving~\eqref{eq:svm_primal} with $\lambda_{1}$. The iterations in~\eqref{eq:alg_svm} and the FISTA algorithm were stopped once the second optimality condition in~\eqref{eq:svm_opt-conds} was approximately met: $\normsq{\by^{*}_{k} - \frac{1}{m}(\bu_{k}-\bb)} \leqslant 10^{-8}$.

Table 1 shows the average CPU run times for the FISTA and accelerated nonlinear PDHG algorithms. The run times for FISTA include the time required to compute the largest singular value of the kernel matrix $\matr{K}$.
\end{comment}

%\subsection{Kernel methods}\label{subsec:kernel}
%We present here accelerated nonlinear PDHG algorithms designed for kernel logistic regression, SVMs without offset and kernel ridge regression. These supervised learning tasks classify or regress with respect to a feature space defined by a positive definite symmetric (PDS) kernel. Concretely, suppose we receive $m$ independent samples $\{(\bv_i,b_i)\}_{i=1}^{m}$, each comprising an input $\bv_i$ from some input space $\mathcal{I}$ and a response variable $b_{i}$. For kernel logistic regression and SVMs without offset the response variable is a label $\{-1,+1\}$, and for kernel ridge regression the response variable is a real number. For these problems, we define a PDS kernel $K \colon \mathcal{I} \times \mathcal{I} \to \R$ via a bounded feature mapping $\bPhi \colon \mathcal{I} \to \Rn$, so that $K(\bv,\bv') = \left\langle \bPhi(\bv),\bPhi(\bv') \right\rangle$ and

%The aim of the kernel methods describe below is to solve the primal minimization problem
%\begin{equation}\label{eq:primal_kernel_general}
%\min_{\bx \in \Rn} \left\{\frac{\lambda}{2}\normsq{\bx} + h(\matr{A}\bx)\right\},
%\end{equation}
%where $\lambda > 0$ is a tuning parameter, $h$ denotes the convex loss function for the model at hand (logistic, hinge or least squared) and $\matr{A}$ denotes an $m\times n$ real matrix constructed from the inputs $\bv_{i}$ and feature mapping $\bPhi$. In general, the matrix $\matr{A}$ may be very difficult or outright impossible to evaluate while computing a kernel value is much cheaper. 


%%%%% LASSO

\subsection{The Lasso}\label{subsec:lasso}
The Lasso is a supervised learning algorithm for regression that aims to identify important features in data sets. Unlike kernel ridge regression, the sparse group Lasso does not make use of PDS kernels. Concretely, suppose we receive $m$ independent samples $\{(\bv_{i},b_{i})\}_{i=1}^{m}$, each comprising an input $\bv_{i}$ from some input space $\mathcal{I}$ and a response variable $b_{i} \in \R$. We map each input to an $n$-dimensional vector of features via a bounded feature mapping $\bPhi\colon \mathcal{I} \to \Rn$ with $\sup_{\bv \in \mathcal{I}}\normtwo{\bPhi(\bv)} < +\infty$. The $m$ vectors of $n$ features are encoded in an $m \times n$ matrix $\matr{A}$ and the response variables are encoded in an $m$-dimensional vector $\bb$. We seek to solve the primal problem
\begin{equation}\label{eq:LASSO_primal}
\inf_{\bx \in \Rn} \left\{\lambda\normone{\bx} + \frac{1}{2m}\normsq{\matr{A}\bx - \bb} \right\},
\end{equation}
where $\lambda > 0$ is a parameter. Here the $\ell_{1}$ penalty promotes sparsity in the solution(s) of~\eqref{eq:LASSO_primal}; that is, the global minimum(s) of~\eqref{eq:LASSO_primal} have a number of entries that are identically zero. The number of zero entries themselves depend on the value of the parameter $\lambda$. We note for this problem that selection rules exist to identify, a priori, a large portion of the non-zero entries of the solution(s) of~\eqref{eq:LASSO_primal} (e.g.,~\cite{ghaoui2010safe}). The forthcoming accelerated nonlinear PDHG method for the Lasso will be able to leverage such selection rules; an example will be shown in Section~\ref{subsec:numerics_lasso}.

The dual problem for the Lasso is given by
\begin{equation}\label{eq:LASSO_dual}
\sup_{\by^{*} \in C_{\lambda}} \left\{- \left\langle \by^{*}, \bb\right\rangle - \frac{m}{2}\normsq{\by^{*}}\right\},
\end{equation}
where $C_{\lambda} = \left\{\by^{*} \in \Rm : \norminf{\matr{A}^{*}\by^{*}} \leqslant \lambda\right\}$. The associated convex-concave saddle-point problem is
\begin{equation}\label{eq:LASSO_saddle}
\inf_{\bx \in \Rn} \sup_{\by^{*} \in \Rm} \left\{\lambda \normone{\bx} + \left\langle\by^{*},\matr{A}\bx - \bb \right\rangle - \frac{m}{2}\normsq{\by^{*}}\right\}.
\end{equation}
Due to the coercivity of the $\ell_1$ norm in the primal problem and the strong convexity of the dual problem, the saddle-point problem~\eqref{eq:LASSO_saddle} admits at least one saddle point. If $(\bx_{s},\by^{*}_{s})$ is a saddle point of~\eqref{eq:LASSO_saddle}, then $\bx_{s}$ is a global minimum of the primal problem~\eqref{eq:LASSO_primal} and $\by^{*}_{s}$ is the unique global minimum of the dual problem~\eqref{eq:LASSO_dual}. Moreover, the saddle point $(\bx_{s},\by^{*}_{s})$ satisfies the optimality conditions
\begin{equation}\label{eq:LASSO_opt-conds}
-\matr{A}^{*}\by^{*}_{s} \in \lambda \partial \normone{\bx_{s}} \quad \mathrm{and} \quad \by^{*}_{s} = \frac{1}{m}(\matr{A}\bx_{s} - \bb).
\end{equation}

\subsubsection*{Accelerated nonlinear PDHG method}
We propose to compute the solution of the Lasso problem using the accelerated nonlinear PDHG method~\eqref{eq:accII_pdhg_alg} with the following choice of norms and Bregman functions:
\[
\normx{\cdot} = \normone{\cdot}, \quad \normys{\cdot} = \normtwo{\cdot}, \quad \phix(\cdot) = \frac{1}{2}\normsq{\cdot}, \quad \mathrm{and} \quad \phiys{\cdot} = \frac{m}{2}\normsq{\cdot}.
\]
With these choices, assumptions (A1)-(A5) hold. In particular, assumption (A5) holds because of the well-known norm equivalence $\sqrt{m}\normtwo{\by^{*}} \geqslant \normone{\by^{*}}$. Moreover, the induced operator norm is the maximum $\ell_2$ norm of the rows of $\matr{A}$, which for the Lasso is the largest Euclidean norm of the feature mapping $\bPhi$ among all inputs, i.e.,
\[
\normop{\matr{A}} = \sup_{\normtwo{\bx} = 1}\norminf{\matr{A}\bx}
= \max_{i \in \{1,\dots,m\}} \sqrt{\sum_{j=1}^{n}A_{ij}^{2}}
= \max_{i \in \{1,\dots,m\}} \normtwo{\bPhi(\bv_i)}.
\]
The strong convexity parameter is $\gamma_{h^{*}} = 1$. For this method, we set $\theta_{0} \in (0,1)$, $\tau_{0} = 1/(2\normop{\matr{A}}^2)$, and $\sigma_{0} = 2$, $\bx_{-1} = \bx_{0} \in \Rn$ and $\by^{*}_{0} \in \Rm$. The corresponding accelerated nonlinear PDHG method for the Lasso then consists of the iterations
\begin{equation}\label{eq:alg_LASSO}
\begin{alignedat}{1}
    \by_{k+1}^{*} &= \argmax_{\by^{*} \in \Rm} \left\{-\frac{m}{2}\normsq{\by^{*}} + \left\langle \by^{*}, \matr{A}(\bx_{k} + \theta_{k}(\bx_{k} - \bx_{k-1})) -\bb\right\rangle - \frac{m}{2\sigma_{k}}\normsq{\by^{*} - \by_{k}^{*}}\right\}, \\
    \bx_{k+1} &= \argmin_{\bx \in \Rn} \left\{\lambda\normone{\bx} + \left\langle \by_{k+1}^{*}, \matr{A}\bx\right\rangle + \frac{1}{2\tau_{k}}\normsq{\bx-\bx_{k}}\right\}, \\
    \theta_{k+1} &= 1/\sqrt{1 + \sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1}, \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k}.
\end{alignedat}
\end{equation}

Both updates $\by_{k+1}^{*}$ and $\bx_{k+1}$ can be computed exactly. The first follows from a short calculation: \todo{FIX}
\[
\by^{*}_{k+1} = (\by_{k}^{*} + \sigma_{k}\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1}))/m)/(1 + \sigma_{k})
\]
The second can be expressed in terms of the soft thresholding operator~\cite{daubechies2004iterative,figueiredo2001wavelet,lions1979splitting}, defined for $j \in \{1,\dots,n\}$, $\bx' \in \Rn$ and $\beta > 0$ by
\[
\argmin_{\bx \in \xcal} \left\{\frac{1}{2}\normsq{\bx-\bx'} + \beta\normone{\bx}\right\} = (\mathrm{shrink}_{1}(\bx',\beta))_{j} = \begin{dcases}
    [\bx']_{j} - \beta &\quad \mathrm{if}\, [\bx']_{j} > \beta, \\
    0 &\quad \mathrm{if}\, |[\bx']_{j}| < \beta, \\
    [\bx']_{j} + \beta &\quad \mathrm{if}\, [\bx']_{j} < -\beta.
\end{dcases}
\]
The second update is
\[
\bx_{k+1} = \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right).
\]

In summary, our accelerated nonlinear PDHG method for solving the Lasso problem~\eqref{eq:LASSO_primal} is as follows. Let $\theta_{0} \in (0,1)$, $\tau_{0} = 1/(2\normop{\matr{A}}^2)$, and $\sigma_{0} = 2$, $\bx_{-1} = \bx_{0} \in \Rn$ and $\by^{*}_{0} \in \Rm$. Then iterate
\begin{equation}\label{eq:alg_lasso}
\begin{dcases}
\by^{*}_{k+1} &= (\by_{k}^{*} + \sigma_{k}(\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1})) - \bb)/m)/(1 + \sigma_{k}) \\
\bx_{k+1} &= \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right) \\
\theta_{k+1} &= 1/\sqrt{1 + \sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1} \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k}
\end{dcases}
\end{equation}
until convergence. According to Prop.~\eqref{prop:acc_sq_algII} and the optimality conditions~\eqref{eq:LASSO_opt-conds}, we have the limits $\lim_{k \to +\infty} \by_{k}^{*} = \by_{s}^{*}$ and $\lim_{k \to +\infty} m\by_{k}^{*} = \matr{A}\bx_{s} - \bb$.

The first limit can be used to identify the zero entries of the global solution(s) of the Lasso problem~\eqref{eq:LASSO_primal}. Indeed, from the first optimality condition~\eqref{eq:LASSO_opt-conds} we have that for any solution $\bx_{s}$ of the Lasso problem~\eqref{eq:LASSO_primal},
\[
\begin{alignedat}{1}
\lambda \partial \normone{\bx_{s}} \ni -\matr{A}^{*}\by_{s}^{*} = \lim_{k \to +\infty} -\matr{A}^{*}\by_{k}^{*}.
\end{alignedat}
\]
For sufficiently large $k$, the magnitude of each entry of $-\matr{A}^{*}\by_{k}^{*}$ will be close to the corresponding entry of $-\matr{A}^{*}\by_{k}^{*}$. Up to some numerical tolerance level, the zero entries of $\bx_{s}$ would then correspond to the entries $-\matr{A}^{*}\by_{k}^{*}$ that are less in magnitude than the parameter $\lambda$.


\subsection{The Lasso}\label{subsec:numerics_lasso}
%After these, we also present some numerical experiments to compare the nonlinear PDHG method~\eqref{eq:alg_lasso} with the current state-of-the-art coordinate-descent based method implemented in glmnet. For the latter, we also implement a so-called selection rule to accelerated the Lasso.
% Mention select rule in the Lasso problem? Make it another subsection in section 5. Then edit this section.

We perform numerical experiments using the accelerated linear PDHG method, the accelerated nonlinear PDHG method~\eqref{eq:alg_lasso}, FISTA, and the Lasso implementation of the glmnet software. We perform here three sets of experiments. In the first set of experiments, we compare the timings required for the convergence of the two PDHG methods and FISTA. For the second set of experiments, we compare again the timings required for the convergence of the two PDHG methods and FISTA, but this time the methods are accelerated using a so-called selection rule~\cite{ghaoui2010safe}. For the third set of experiments, we compare the timings required for the convergence of the accelerated nonlinear PDHG method~\eqref{eq:alg_lasso} aided by a selection rule and the Lasso implementation of the glmnet software, the latter which incorporates a selection rule as well.

For the accelerated linear PDHG method, we calculate the largest singular value $s(\matr{A})$ of the feature matrix $\matr{A}$ and compute the iterates
\[
\begin{dcases}
\by^{*}_{k+1} &= (\by_{k}^{*} + \sigma_{k}(\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1})) - \bb)/(1 + m\sigma_{k}) \\
\bx_{k+1} &= \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right) \\
\theta_{k+1} &= 1/\sqrt{1 + m\sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1} \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k},
\end{dcases}
\]
with $\theta_{0} = 0$, $\tau_{0} = m/(2s(\matr{A})^{2})$ and $\sigma_{0} = 2/m$. For both the linear and nonlinear PDHG methods, we set $\bx_{-1} = \bx_{0} = \boldsymbol{0}$ and $\by_{0}^{*} = \bb$. We compute the time required for the convergence in the dual variable $\by_{k}^{*}$ and also the time required for convergence in the average dual variable $\bY_{k}^{*}$ as defined in Prop.~\ref{prop:acc_sq_algII}:
\[
\bY_{K}^{*} = \frac{1}{T_{K}}\sum_{k=1}^{K} \frac{\tau_{k-1}}{\tau_{0}} \by_{k}^{*} \quad \text{where} \quad T_{K} = \sum_{k=1}^{K}\frac{\tau_{k-1}}{\tau_{0}}.
\]
In both methods, the iterations were stopped once $\normsq{\by^{*}_{k+1} - \by^{*}_{k}} \leqslant 10^{-8}$ and $\normsq{\bY^{*}_{K+1} - \bY^{*}_{K}} \leqslant 10^{-8}$. For the FISTA method, we compute the iterates
\[
\begin{dcases}
\bw_{k} &= \bx_{k} + \beta_{k}(\bx_{k} - \bx_{k-1})\\
\bx_{k+1} &= \text{shrink}_{1}(\bw_{k} - \tau\matr{A}^{*}(\matr{A}\bw_{k} - \bb)/m,\lambda\tau),\\
t_{k+1} &= \frac{1 + \sqrt{1 + 4t_{k}^{2}}}{2},\\
\beta_{k+1} &= \frac{(t_{k}-1)}{t_{k+1}}.
\end{dcases}
\]
where we set $\tau = m/S(\matr{A})^2$, $\bx_{-1} = \bx_{0} = \boldsymbol{0}$ and $t_{0} = \beta_{0} = 0$. We compute the time required for convergence in the variable $\bu_{k}$. The iterations in FISTA were stopped once $\normsq{\bx_{k+1} - \bx_{k}} \leqslant 10^{-8}$.

In the second and third set of numerical experiments presented here, we use a so-called selection rule to accelerate the computations of both PDHG methods and FISTA. Selection rules aim to identify a priori a large portion of the non-zero entries of the solution(s) of the Lasso problem. We use here the following selection rule for the Lasso problem~\eqref{eq:LASSO_primal}, due to~\cite{ghaoui2010safe}. Denote the columns of the matrices $\matr{A}$ by $\ba_{j}$ for $j \in \{1,\dots,n\}$. Let $\by_{s}^{*}(\lambda_{0})$ denote the unique solution of the dual Lasso problem~\eqref{eq:LASSO_dual} with parameter $\lambda_{0}$. Fix $0 < \lambda \leqslant \lambda_{0}$ and define the constants
\[
\gamma = \frac{\left|\left\langle \by_{s}^{*}(\lambda_{0}),\bb \right\rangle \right|^{2}}{2m\normsq{\by_{s}^{*}(\lambda_{0})}}\left(1 - \max{\left(0,\frac{m^2\lambda\normsq{\by_{s}^{*}(\lambda_{0})}}{\left|\left\langle\by_{s}^{*}(\lambda_{0}),\bb \right\rangle\right|\norminf{\matr{A}^{*}\by_{s}^{*}(\lambda_{0})}}-1\right)}\right) \quad \text{and} \quad D = \left[\normsq{\bb} - 2m\gamma\right]^{1/2}.
\]
Finally, let $F$ denote the objective function of the dual Lasso problem~\eqref{eq:LASSO_dual} and define the function $P\colon \Rn \mapsto \R$ as
\[
P(\ba) = 
\begin{dcases}
&\frac{1}{m}\left(D\normtwo{\ba} - \left\langle \bb,\ba \right\rangle\right)\; \text{if} \; \normtwo{\ba}\normsq{\nabla F(\by_{s}^{*}(\lambda_{0}))} \geqslant D\left\langle \nabla F(\by_{s}^{*}(\lambda_{0})),\ba \right\rangle, \\
&\left\langle \by_{s}^{*}(\lambda_{0}), \ba \right\rangle - \left[\left(D^{2}-\normsq{\nabla F(\by_{s}^{*}(\lambda_{0}))}\right)\left(\normsq{\ba} - \frac{\left|\left\langle \nabla F(\by_{s}^{*}(\lambda_{0})),\ba \right\rangle \right|^{2}}{\normsq{\nabla F(\by_{s}^{*}(\lambda_{0}))}}\right)\right]^{1/2}\; \text{otherwise.}
\end{dcases}
\]
The selection rule due to~\citet{ghaoui2010safe} states that if $\max{(P(\ba_{j}),P(-\ba_{j}))} < \lambda$, then the $j^{\text{th}}$-component of the global solution(s) of the Lasso problem~\eqref{eq:LASSO_primal} with parameter $\lambda$ is zero.


\subsubsection*{Numerical results I}
\todo{Complete}

\subsubsection*{Numerical results II}
\todo{Complete. For this problem, we set $\lambda_{0} = \norminf{\matr{A}^{*}\bb}/m$ and take half its value for $\lambda$.}



\subsubsection*{Numerical results III}
\todo{Complete. For this problem, we use the solution path generated from glmnet starting at $\norminf{\matr{A}^{*}\bb}/m$.}

%For this experiment, we set $\alpha = 0.5$ and used the dimensions $(m,d) = (1000, 100000)$, $(m,d) = (2500, 40000)$, and $(m,d) = (10000, 10000)$ for the samples $(\bv_{1},\dots,\bv_{m})$.  The dimension of the primal problem~\eqref{eq:enrlr_primal} is $n = d$. For each pair $(m,d)$, we used the correlation coefficient $r \in \{0.25,0.75\}$, for a total of six simulations. In each simulation, we ran glmnet to let it generate (using the default settings) a decreasing sequence of 100 tuning parameters $\{\lambda_{l}\}_{l=1}^{100}$. We then let glmnet solve the elastic net linear regression problem~\eqref{eq:enrlr_primal} sequentially for each $\lambda_{l}$ using the solution found for~\eqref{eq:enrlr_primal} with tuning parameter $\lambda_{l}$ as the initial solution for~\eqref{eq:enrlr_primal} with tuning parameter $\lambda_{l+1}$. The initial values $\bx_{0} = \boldsymbol{0}$ and $\by_{-1}^{*} = \by_{0}^{*} = \bb$ were used for solving~\eqref{eq:enrlr_primal} with $\lambda_{1}$. We then used the same sequence of tuning parameters $\{\lambda_{l}\}_{l=1}^{m}$ and strategy as above to solve~\eqref{eq:enrlr_primal} sequentially for each $\lambda_{l}$ with our implementation of the nonlinear PDHG method~\eqref{eq:alg_enrlr} and FISTA. The iterations in~\eqref{eq:alg_enrlr} and the FISTA method were stopped once the optimality conditions~\eqref{eq:enrlr_opt-conds} were approximately met: $\normsq{\by^{*}_{k} - \frac{1}{m}(\matr{A}\bx_{k} - \bb)} \leqslant 10^{-8}$ and \todo{Change?}
% \[
% -\frac{1}{\lambda}\left(2\matr{A}^{*}\by_{k}^{*} + \lambda\bx_{k}\right)_{i} \in 
% \begin{dcases}
% (-1.0001,-0.9999) &\quad \mathrm{if}\, (\bx_{k})_i > 0\\  
% [-0.9999,0.9999] &\quad \mathrm{if}\, (\bx_{k})_i = 0\\  
% (0.9999,1.0001) &\quad \mathrm{if}\, (\bx_{k})_i < 0.
% \end{dcases}
% \]

% Table 3 shows the average CPU run times for the glmnet, FISTA, and accelerated nonlinear PDHG methods. The run times for FISTA include the time required to compute the largest singular value of the matrix $\matr{A}$.



% \subsection{The Lasso}
% For this experiment, we used the dimensions $(m,d) = (1000, 100000)$, $(m,d) = (2500, 40000)$, and $(m,d) = (10000, 10000)$ for the samples $\{\bv_{1},\dots,\bv_{m}\}$. The dimension of the primal problem~\eqref{eq:LASSO_primal} is $n = d$. For each pair $(m,d)$, we used the correlation coefficient $r \in \{0.25,0.75\}$, for a total of six simulations. In each simulation, we ran glmnet to let it generate (using the default settings) a decreasing sequence of 100 tuning parameters $\{\lambda_{l}\}_{l=1}^{100}$. We then let glmnet solve the Lasso~\eqref{eq:LASSO_primal} sequentially for each $\lambda_{l}$ using the solution found for~\eqref{eq:LASSO_primal} with tuning parameter $\lambda_{l}$ as the initial solution for~\eqref{eq:LASSO_primal} with tuning parameter $\lambda_{l+1}$. The initial values $\bx_{0} = \boldsymbol{0}$ and $\by_{-1}^{*} = \by_{0}^{*} = \bb$ were used for solving~\eqref{eq:LASSO_primal} with $\lambda_{1}$. We then used the same sequence of tuning parameters $\{\lambda_{l}\}_{l=1}^{m}$ and strategy as above to solve~\eqref{eq:LASSO_primal} sequentially for each $\lambda_{l}$ with our implementation of the nonlinear PDHG method~\eqref{eq:alg_LASSO} and FISTA. The initial parameters $\theta_{0} = \frac{1}{2}$ and $\tau_{0} = m/(2\normop{\matr{A}^2})$ were used in all simulations. The iterations in~\eqref{eq:alg_LASSO} and the FISTA method were stopped once the optimality conditions~\eqref{eq:LASSO_opt-conds} were approximately met: $\normsq{\by^{*}_{k} - \frac{1}{m}(\matr{A}\bx_{k} - \bb)} \leqslant 10^{-8}$ and \todo{change}?
% \[
% -\frac{1}{\lambda}\left(\matr{A}^{*}\by_{k}^{*}\right)_{i} \in
% \begin{dcases}
% (-1.0001,-0.9999) &\quad \mathrm{if}\, (\bx_{k})_i > 0\\  
% [-0.9999,0.9999] &\quad \mathrm{if}\, (\bx_{k})_i = 0\\  
% (0.9999,1.0001) &\quad \mathrm{if}\, (\bx_{k})_i < 0.
% \end{dcases}
% \]

% Table 4 shows the average CPU run times for the glmnet, FISTA, and accelerated nonlinear PDHG methods. The run times for FISTA include the time required to compute the largest singular value of the matrix $\matr{A}$.

%% Times for computing the matrix must be the same as before... do not report it in a bracket...
%%%%%

%%%%%

\begin{comment}
\subsection{Notation}\label{subsec:notation}
Throughout this work, $(\xcal,\normx{\cdot})$ and $(\ycal,\normy{\cdot})$ denote two real reflexive Banach spaces. We assume that $\xcal$ and $\ycal$ are real reflexive Banach spaces endowed with corresponding norms $\normx{\cdot}$ and $\normy{\cdot}$. The interior of a non-empty subset $C$ of $\xcal$ or $\ycal$ is denoted by $\interior{~C}$. The class of proper, convex and lower semicontinuous functions defined on $\xcal$ and $\ycal$ are denoted by $\gmxcal$ and $\gmycal$. The dual spaces of all continuous linear functionals defined on $\xcal$ and $\ycal$ are denoted by $\xcal^*$ and $\ycal^*$. For a linear functional $\bx^* \in \xcal^*$ and an element $\bx \in \xcal$, the bilinear form $\left\langle \bx^*,\bx \right\rangle$ gives the value of $\bx^*$ at $\bx$. Likewise, for a linear functional $\by^* \in \ycal^*$ and an element $\by \in \ycal$, the bilinear form $\left\langle \by^*,\by \right\rangle$ gives the value of $\by^*$ at $\by$. The norms associated to $\xcal^*$ and $\ycal^*$ are defined as
\[
\normxs{\bx^*} = \sup_{\normx{\bx} = 1} \left\langle \bx^*,\bx \right\rangle \quad \mathrm{and} \quad \normys{\by^*} = \sup_{\normy{\by} = 1} \left\langle \by^*,\by \right\rangle.
\]
Let $\matr{A}\colon \xcal \to \ycal$ denote a bounded linear operator. Its corresponding adjoint operator $\matr{A}^*\colon \ycal^* \to \xcal^*$ is defined so as to satisfy
\begin{equation*}
    \left\langle \matr{A}^*\by^*,\bx \right\rangle = \left\langle \by^*,\matr{A}\bx \right\rangle
\end{equation*}
for every $\bx \in \xcal$ and $\bys \in \ycal^*$. The operator norm associated to $\matr{A}$ is defined as
\begin{equation*}
    \normop{\matr{A}} = \sup_{\normx{\bx} = 1} \normy{\matr{A}\bx} = \normop{\matr{A}^*} = \sup_{\normys{\by^*} = 1}\normxs{\matr{A}^*\by^*}.
\end{equation*}
\end{comment}

\begin{comment}
We wish to identify which of the $n$ features best describe the observed response variables. A common approach to do so is to minimize a trade-off between the empirical mean squared error and an $\ell_{1}$ penalty:
\begin{equation}\label{eq:intro_lasso}
\inf_{\bx \in \Rn} \left\{\lambda\normone{\bx} + \frac{1}{2m}\normsq{\matr{A}\bx - \bb} \right\}.
\end{equation}
This feature selection method is called the Lasso (least absolute shrinkage and selection operator). Here, $\lambda > 0$ is a tuning parameter. The solution to the Lasso problem does not have a closed-form solution, but we can approximate it using the following accelerated linear PDHG method~\cite[Algorithm 8 and Remark 5.3]{chambolle2016introduction}: Let $\bx_{-1} = \bx_{0} \in \Rn$ and $\by^{*}_{0} \in \Rm$ denote a set of initial values, let $s(\matr{A})$ denote the largest singular value of the matrix $\matr{A}$, and define the stepsize parameters $\theta_{0} = 1$, $\tau_{0} = m/2(s(\matr{A})^{2})$ and $\sigma = 2/m$. The accelerated linear PDHG method computes the iterates \todo{FIX}
\begin{equation}\label{eq:intro_lasso-alg}
\begin{alignedat}{1}
    \by_{k+1}^{*} &= \argmin_{\by^{*} \in \Rm} \left\{\frac{m}{2}\normsq{\by^{*}} - \left\langle \by^{*}, \matr{A}(\bx_{k} + \theta_{k}(\bx_{k} - \bx_{k-1})) -\bb\right\rangle + \frac{1}{2\sigma_{k}}\normsq{\by^{*} - \by_{k}^{*}}\right\}, \\
    \bx_{k+1} &= \argmin_{\bx \in \Rn} \left\{\lambda\normone{\bx} + \left\langle \by_{k+1}^{*}, \matr{A}\bx\right\rangle + \frac{1}{2\tau_{k}}\normsq{\bx-\bx_{k}}\right\}, \\
    \theta_{k+1} &= 1/\sqrt{1 + m\sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1}, \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k},
\end{alignedat}
\end{equation}
until convergence. Both updates $\by^{*}_{k+1}$ and $\bx_{k+1}$ can be computed exactly. The first follows from a short calculation:
\[
\by^{*}_{k+1} = \frac{1}{1+m\sigma_{k}}(\by_{k}^{*} + \sigma_{k}\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1})) - \bb).
\]
The second can be expressed in terms of the soft thresholding operator~\cite{daubechies2004iterative,figueiredo2001wavelet,lions1979splitting}, defined for $j \in \{1,\dots,n\}$, $\bx' \in \Rn$ and $\beta > 0$ by
\[
\argmin_{\bx \in \xcal} \left\{\frac{1}{2}\normsq{\bx-\bx'} + \beta\normone{\bx}\right\} = (\mathrm{shrink}_{1}(\bx',\beta))_{j} = \begin{dcases}
    [\bx']_{j} - \beta &\quad \mathrm{if}\, [\bx']_{j} > \beta, \\
    0 &\quad \mathrm{if}\, |[\bx']_{j}| < \beta, \\
    [\bx']_{j} + \beta &\quad \mathrm{if}\, [\bx']_{j} < -\beta.
\end{dcases}
\]
The second update is
\[
\bx_{k+1} = \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right).
\]
Hence the updates are
\begin{equation}\label{eq:intro_lasso-alg_explicit}
\begin{dcases}
    \by_{k+1}^{*} &= \left(\by_{k}^{*} + \sigma_{k}(\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1})) - \bb)\right)/(1+m\sigma_{k}), \\
    \bx_{k+1} &= \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right), \\
    \theta_{k+1} &= 1/\sqrt{1 + m\sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1} \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k}.
\end{dcases}
\end{equation}

The updates in~\eqref{eq:intro_lasso-alg_explicit} are easy to evaluate; they can be computed exactly in $O(mn)$ operations. Moreover, for the choice above of the stepsize parameters $\tau$ and $\sigma$, the sequence of iterates in the dual variable $\{\by_{k}^{*}\}_{k=1}^{+\infty}$ strongly converges to the unique solution of the dual problem associated to the Lasso problem~\eqref{eq:intro_lasso}. The convergence rate is sublinear rate $O(1/k^{2})$ in the number of iterations~\cite{chambolle2016ergodic}, which is the best possible achievable rate of convergence for this problem in the Nesterov class of optimal first-order methods~\cite{Nesterov2018}. Identifying the zero entries of the global solution(s) to the Lasso problem~\eqref{eq:intro_lasso} can be done using the optimal condition for the Lasso problem~\eqref{eq:intro_lasso}.

Attaining the optimal rate of convergence requires a precise estimate of the largest singular value $s(\matr{A})$ of the matrix $\matr{A}$. This quantity, however, takes on the order of $O(\min(m^2n,mn^2))$ operations to compute~\cite{hastie2009elements}. This high computational cost makes it essentially impossible to estimate the largest singular value for high-dimensional matrices. Line search methods and other heuristics are sometimes used to bypass this problem, but they come at the cost of significantly slowing down the convergence of the linear PDHG method. This problem is common to most first-order optimization methods for regression and classification problems in machine learning.

Thus, despite being flexible and easy to implement, the linear PDHG method is often impractical for solving large-scale problems in machine learning. This paper introduces accelerated nonlinear PDHG methods that avoid this issue and achieve an optimal rate of convergence with stepsize parameters that are simple to compute. 
% TODO: Can cut a lot of text here bu going straight to the method.
As an illustration, we show in Sections~\ref{subsec:accIII} and~\ref{subsec:lasso} that for the following choice of matrix norm
\[
\normop{\matr{A}} = \max_{j \in \{1,\dots,n\}} \sqrt{\sum_{i=1}^{m}A_{ij}^{2}},
\]
stepsize parameters $\theta_{0} \in (0,1)$, $\tau_{0} = 1/(2\normop{\matr{A}}^2)$ and $\sigma_{0} = 2$, and initial values $\bx_{-1} = \bx_{0} \in \Rn$ and $\by^{*}_{0} \in \Rm$, the accelerated nonlinear PDHG method \todo{CORRECT}
\begin{equation}\label{eq:intro_lasso-alg-alt}
\begin{dcases}
\by^{*}_{k+1} &= (\by_{k}^{*} + \sigma_{k}(\matr{A}(\bx_{k} + \theta_{k}(\bx_{k}-\bx_{k-1}))/m - \bb))/(1 + \sigma_{k}) \\
\bx_{k+1} &= \mathrm{shrink}_{1}\left(\bx_{k} - \tau_{k}\matr{A}^{*}\by^{*}_{k+1},\lambda\tau_{k}\right) \\
\theta_{k+1} &= 1/\sqrt{1 + \sigma_{k}}, \quad \tau_{k+1} = \tau_{k}/\theta_{k+1} \quad \mathrm{and} \quad \sigma_{k+1} = \theta_{k+1}\sigma_{k}
\end{dcases}
\end{equation}
yields a sequence of iterates for the dual variable $\{\by_{k}^{*}\}_{k=1}^{+\infty}$ that strongly converges to the unique solution of the dual problem associated to the Lasso problem~\eqref{eq:intro_lasso}. This rate of convergence is also optimal at a sublinear $O(1/k^2)$ in the number of iterations. In contrast to the linear method~\eqref{eq:intro_lasso-alg_explicit}, the stepsize parameters and operations in the nonlinear method~\eqref{eq:intro_lasso-alg-alt} can all be computed in optimal $\Theta(mn)$ steps. This is because all parameters in method~\eqref{eq:intro_lasso-alg-alt} depend on the operator norm $\normop{\matr{A}} = \max_{j \in \{1,\dots,n\}} \sqrt{\sum_{i=1}^{m}A_{ij}^{2}}$, which takes on the order of $\Theta(mn)$ operations to compute. Although method~\eqref{eq:intro_lasso-alg-alt} introduces an extra factor of $1/m$ in the parameter $\theta$ and in the first update $\by^{*}_{k+1}$, which influences the number of iterations needed for convergence, numerical experiments that we perform in Section~\ref{sec:numerics} suggest that the nonlinear method~\eqref{eq:intro_lasso-alg-alt} nonetheless converges much faster than its linear counterpart~\eqref{eq:intro_lasso-alg} when the dimension $n$ is very large. %TODO Provide a reference to a table.
\end{comment}

\begin{comment}
To illustrate this point, consider the following standard ridge regression problem in machine learning: Suppose we receive $m$ independent samples, each comprising an $n$-dimensional vector of features and a response variable. The samples are encoded in an $m \times n$ real matrix $\matr{A}$ whose columns are the features and a response vector $\bb \in \Rm$. We assume in this example that the response variable is linear and that the features are highly correlated. A common approach to fit the samples is to minimize a trade-off between the empirical squared-loss and a squared $l_2$-norm:
\begin{equation}\label{eq:intro_ridge-reg}
\inf_{\bx \in \Rn} \left\{\frac{\lambda}{2}\normsq{\bx} + \frac{1}{2m}\normsq{\matr{A}\bx - \bb} \right\},
\end{equation}
where $\lambda > 0$ is a free parameter. The solution to this problem is
\[
\bx_{sol} = \left(\matr{A}^{*}\matr{A} + \lambda m \matr{I}_{n\times n}\right)^{-1}\matr{A}^{*}\bb.
\]
Computing the solution $\bx_{sol}$ this way is impractical for large matrices because it takes on the order of $O(\min{(mn^2 + n^3, m^2n + m^3}))$ operations to perform matrix multiplication and matrix inverse calculations~\cite{mohri2018foundations}. % TODO: Verify number of operations + harmonize.
\end{comment}



\subsection{Kernel logistic regression}
We perform numerical experiments using the accelerated nonlinear PDHG method~\eqref{eq:alg_klr} and FISTA. We do not use the accelerated linear PDHG method for kernel logistic regression because it does not lead to an explicit algorithm. For the nonlinear PDHG method, we set $\bu_{-1} = \bu_{0} = \boldsymbol{0}$ and $[\by_{0}^{*}]_{i} = 0.5/m$ for each $i \in \{1,\dots,m\}$. We compute the time required for convergence in the dual variable $\by_{k}^{*}$ and also the time required for convergence in the average dual variable $\bY_{k}^{*}$ as defined in Prop.~\ref{prop:acc_sq_algII_var}:
\[
\bY_{K}^{*} = \frac{1}{T_K}\sum_{k=1}^{K}\frac{1}{\theta^{k-1}} \by_{k}^{*} \quad \text{where} \quad T_{K} = \sum_{k=1}^{K} \frac{1}{\theta^{k-1}} = \frac{1-\theta^{K}}{(1-\theta)\theta^{K-1}}.
\]
The iterations were stopped once $\normtwo{\by^{*}_{k+1} - \by^{*}_{k}} \leqslant 10^{-4}\normtwo{\by^{*}_{k+1}}$ and $\normtwo{\bY^{*}_{K+1} - \bY^{*}_{K}} \leqslant 10^{-4}\normtwo{\bY^{*}_{K+1}}$. 

For the FISTA method, we evaluate the largest singular value $s(\matr{K}_{\text{Logistic}})$ of the kernel matrix $\matr{K}_{\text{Logistic}}$ and compute the iterates
\[
\begin{dcases}
\bw_{k} &= \bu_{k} + \beta_{k}(\bu_{k} - \bu_{k-1}),\\
[\bv_{k}]_{i} &= 1/(m + m\exp{(-[\bw_{k}]_{i})}) \quad \text{for} \quad i \in \{1,\dots,m\},\\
\bu_{k+1} &= (\bw_{k} - \tau\matr{K}_{\text{Logistic}}\bv_{k})/(1+\lambda\tau)\\
t_{k+1} &= \frac{1-qt_{k}^{2} + \sqrt{(1-qt_{k}^{2})^{2} + 4t_{k}^{2}}}{2},\\
\beta_{k+1} &= \frac{(t_{k}-1)(1+\tau\lambda(1-t_{k+1}))}{t_{k+1}},
\end{dcases}
\]
where we set $\tau = 4m/s(\matr{K}_{\text{Logistic}})^{2}$, $q = \lambda\tau/(1+\lambda\tau)$, $\bu_{-1} = \bu_{0} = \boldsymbol{0}$ and $t_{0} = \beta_{0} = 0$. We compute the time required for convergence in the variable $\bu_{k}$. The iterations were stopped once $\normtwo{\bu_{k+1} - \bu_{k}} \leqslant 10^{-4}\normtwo{\bu_{k+1}}$.

\subsubsection*{Numerical results}
\todo{Update script and present the numerical results...}

\subsection{Kernel ridge regression}
We perform numerical experiments using the accelerated linear PDHG method, the nonlinear PDHG method~\eqref{eq:alg_krr} and FISTA. For the accelerated linear PDHG method, we evaluate the largest singular value $s(\matr{K}_{\text{Ridge}})$ of the kernel matrix $\matr{K}_{\text{Ridge}}$ and compute the iterates
\[
    \begin{dcases}
    \bu_{k+1} &= \left(\bu_{k} - \tau\matr{K}_{Ridge}(\by_{k}^{*} + \theta(\by_{k}^{*} - \by_{k-1}^{*}))\right)/(1 + \lambda\tau),\\ 
    \by_{k+1}^{*} &= \left(\by_{k}^{*} + \sigma(\bu_{k+1} - \bb)\right)/(1+m\sigma),\\
    \end{dcases}
\]
where the step size parameters are
\[
\theta = 1 - \frac{\lambda m}{2s(\matr{K}_{\text{Ridge}})^{2}}\left(\sqrt{1 + \frac{4s(\matr{K}_{\text{Ridge}})^{2}}{\lambda m}} - 1\right), \quad \tau = \frac{(1-\theta)}{\lambda\theta} \quad \mathrm{and} \quad \sigma = \frac{1-\theta}{m\theta}.
\]
For both the linear and nonlinear PDHG methods, we set $\bu_{-1} = \bu_{0} = 0$ and $\by_{0}^{*} = \bb$. We compute the time required for convergence in the dual variable $\by_{k}^{*}$ and also the time required for convergence in the average dual variable $\bY^{*}$ as defined in Prop.~\ref{prop:acc_sq_algIII}:
\[
\bY_{K}^{*} = \frac{1}{T_K}\sum_{k=1}^{K}\frac{1}{\theta^{k-1}} \by_{k}^{*} \quad \text{where} \quad T_{K} = \sum_{k=1}^{K} \frac{1}{\theta^{k-1}} = \frac{1-\theta^{K}}{(1-\theta)\theta^{K-1}}.
\]
In both methods, the iterations were stopped once $\normtwo{\by^{*}_{k+1} - \by^{*}_{k}} \leqslant 10^{-4}\normtwo{\by^{*}_{k+1}}$ and $\normtwo{\bY^{*}_{K+1} - \bY^{*}_{K}} \leqslant 10^{-4}\normtwo{\bY^{*}_{K+1}}$. For the FISTA method, we compute the iterates
\[
\begin{dcases}
\bw_{k} &= \bu_{k} + \beta_{k}(\bu_{k} - \bu_{k-1})\\
\bu_{k+1} &= (\bw_{k} - \tau\matr{K}_{\text{Ridge}}(\bw_{k}-\bb)/m)/(1+\lambda\tau)\\
t_{k+1} &= \frac{1-qt_{k}^{2} + \sqrt{(1-qt_{k}^{2})^{2} + 4t_{k}^{2}}}{2},\\
\beta_{k+1} &= \frac{(t_{k}-1)(1+\tau\lambda(1-t_{k+1}))}{t_{k+1}},
\end{dcases}
\]
where we set $\tau = m/s(\matr{K}_{\text{Ridge}})^{2}$, $q = \lambda\tau/(1+\lambda\tau)$, $\bu_{-1} = \bu_{0} = \boldsymbol{0}$ and $t_{0} = \beta_{0} = 0$. We compute the time required for convergence in the variable $\bu_{k}$. The iterations were stopped once $\normtwo{\bu_{k+1} - \bu_{k}} \leqslant 10^{-4}\normtwo{\bu_{k+1}}$.



\subsubsection*{Numerical results}
TBC.


\todo{Update the script and present the numerical results.}


%We perform two sets of experiments for $\ell_{1}$-constrained logistic regression In the first experiment, 

%In the second experiment, we draw $m$ independent samples $(\bu_{1},\dots,\bu_{m})$ iid from a $d$-Gaussian distribution with zero mean and unit variance but where each sample has approximately only 10\% coefficients set to zero. We generate this data in MATLAB using the command \textit{sprandn(m,d,0.1)}. We draw the labels $(b_{1},\dots,b_{m})$ uniformly at random from $\{-1,+1\}^{m}$ and set $\lambda = 1$ as before. We choose the number of samples to be smaller than then number of features, with $m = 10000$, and $d = 250,000$, $500,000$, $750,000$, $1,000,000$, $1,250,000$ and $1,500,000$.

% TODO: Can we do better? I would generate data as described below, but it is too slow in MATLAB.....

% In the second experiment, we generate linear synthetic data according to the methodology outlined in~\citet[Section 3 and 4]{bertsimas2020sparse}. Specifically, we draw $m$ independent samples $(\bv_{1},\dots,\bv_{m})$ from a $d$-dimensional Gaussian distribution with mean $\boldsymbol{0}$ and covariance matrix $\matr{\Sigma}$ defined component-wise by $\Sigma_{ij} = r^{|i-j|}$ for $r \in (0,1)$. We randomly draw a weight vector $\bx_{\mathrm{true}} \in \{-1,0,1\}$ where only 1\% of the coefficients are nonzero. We draw $z_{i}$, $i \in \{1,\dots,m\}$ independent identically distributed noise components from a normal distribution with zero mean and signal-to-noise ratio equal to one, so that $\normtwo{\bz} = \normtwo{\matr{A}\bx_{\mathrm{true}}}$. Finally, we compute the labels $\{-1,+1\}^{m}$ of each sample via
% \[
% b_{i} = 
% \begin{dcases}
% +1 &\quad \mathrm{if}\, \sign{\left(\left\langle \bx_{\mathrm{true}},\bv_{i} \right\rangle + z_i\right)} \geqslant 0, \\
% -1 &\quad \mathrm{otherwise}.
% \end{dcases}
% \]
% For this experiment, we set $r = 0.75$, $m = 10000$, and $d = 25,000$, $50,000$, $75,000$, $100,000$, $125,000$ and $150,000$.

% ~\eqref{eq:intro_ridge-reg-alg} with initial values $\bx_{0} \in \Rn$ and $\by_{-1} = \by_{0} = \Rm$ and stepsize parameters $\theta$, $\tau$ and $\sigma$ estimated from the matrix norm
% \[
% \norm{\matr{A}}_{2,\infty} = \max_{i \in \{1,\dots,m\}} \sqrt{\sum_{j=1}^{m}A_{ij}^{2}},
% \]
% via
% \[
% \theta = 1 - \frac{\lambda}{2\norm{\matr{A}}_{2,\infty}^{2}}\left(\sqrt{1 + \frac{4\norm{\matr{A}}^{2}_{2,\infty}}{\lambda}} - 1\right), \quad \tau = \frac{(1-\theta)}{\lambda\theta} \quad \mathrm{and} \quad \sigma = \frac{1-\theta}{m\theta},
% \]
%strongly converges to the unique solution of the ridge regression problem~\eqref{eq:intro_ridge-reg}. The convergence rate is $O(\theta^{k})$ in the number of iterations $k$, which is linear is optimal in the Nesterov class of optimal first-order methods. In contrast to the linear PDHG method, the stepsize parameters and operations in the nonlinear method can all be computed in optimal $\Theta(mn)$ steps. This is because all the stepsize parameters are estimated from the matrix norm $\norm{\matr{A}}_{2,\infty}$, which takes on the order of $\Theta(mn)$ operations to compute. 

%The apparent downside is that the convergence rate, which depends on the stepsize parameter $\theta$, is larger for the nonlinear PDHG method than for the linear PDHG method. This implies that the nonlinear PDHG method requires more iterations than the linear PDHG method to converge. As the following numerical experiment shows, however, the [...] \todo{Complete -- Need reference for estimation of ridge parameter when $ n >> m$, then use a lower bound on that coefficient.}

%Nonetheless, numerical experiments that we perform in Section~\ref{sec:numerics} suggest that the nonlinear method takes significantly less time to arrive at an approximate solution than its linear counterpart when the dimension $n$ is large. \todo{Make this concrete -- add a table of timings here. This should be convincing. Try to cut some fluff or add a header or two.}

